A Comparison of Neural Network Architectures for Data-Driven Reduced-Order Modeling

The popularity of deep convolutional autoencoders (CAEs) has engendered new and effective reduced-order models (ROMs) for the simulation of large-scale dynamical systems. Despite this, it is still unknown whether deep CAEs provide superior performance over established linear techniques or other network-based methods in all modeling scenarios. To elucidate this, the effect of autoencoder architecture on its associated ROM is studied through the comparison of deep CAEs against two alternatives: a simple fully connected autoencoder, and a novel graph convolutional autoencoder. Through benchmark experiments, it is shown that the superior autoencoder architecture for a given ROM application is highly dependent on the size of the latent space and the structure of the snapshot data, with the proposed architecture demonstrating benefits on data with irregular connectivity when the latent space is sufficiently large.

==> dead.tex <==
\subsection{Coarsening}
Now that convolution on graphs has been discussed, it is important to discuss how a graph can be meaningfully coarsened so that a useful downsampling procedure can be defined.  Since the ChebNet graph convolution is naturally size-preserving, this requires an additional step at each layer of the GCAE whereby graph signals are aggregated and projected to the next coarse level.

Atomically, many graph reduction schemes can be viewed as generating a sequence of subgraphs $\mathcal{G}_1 \supset \mathcal{G}_2 ... \supset \mathcal{G}_n$ of the graph $\mathcal{G}_0$ through the recursion (c.f. \cite{loukas2019})
\[\bb{A}_\ell =  \bb{P}_\ell^\mp\bb{A}_{\ell-1}\bb{P}_\ell^+, \qquad \bb{x}_\ell = \bb{P}_\ell \bb{x}_{\ell-1}, \]
where $\bb{P}_\ell\in\mathbb{R}^{N_{\ell} \times N_{\ell-1}}$ with $N_{\ell} < N_{\ell-1}$, $\bb{P}_\ell^+ = (\bb{P}_\ell^\top \bb{P}_\ell)^{-1}\bb{P}_\ell^\top$ denotes the pseudoinverse of $\bb{P}_\ell$ and $\bb{P}_\ell^\mp$ denotes the transpose of $\bb{P}_\ell^+$.  Moreover, if $\bb{P}_\ell$ is a surjective mapping of the nodes and the induced subgraph $\mathcal{G}_{\ell}$ of $\mathcal{G}_{\ell-1}$ is connected, $\bb{P}_\ell$ is said to be a coarsening matrix and it can be shown that $\bb{P}_\ell^+ = \bb{P}_\ell^\top \bb{D}_\ell^{-2}$ where $\bb{D}_{\ell,ii} = \|\bb{P}_{\ell,i}\|_2$ (see \cite[Proposition 6]{loukas2019}).  Therefore, if valid coarsening matrices $\bb{P}_\ell$ can be computed efficiently, it follows that both coarsening and lifting signals on subgraphs can be accomplished in linear time.  In particular, note that both $\bb{P}_{\ell}$ and $\bb{P}^+_\ell$ are sparse matrices with only $N_{\ell-1}$ nonzero entries, so that coarsening $\bb{x}_\ell = \bb{P}_{\ell}\bb{x}_{\ell-1}$ or lifting $\tilde{\bb{x}}_{\ell-1} = \bb{P}_\ell^+\tilde{\bb{x}}_\ell$ depend linearly on the number of nodes in $\mathcal{G}_{\ell-1}$.

In principle, any coarsening technique can be used to generate the sequence of subgraphs and coarsening matrices necessary for building a graph autoencoder, although there may be some which are more suitable than others.  Presently, we consider the fast and relatively simple ``heavy edge matching'' technique of \cite{karypis1998}.  In particular, recall that a \emph{matching} of the graph $\mathcal{G}$ is a set of edges no two of which share an incident vertex.  As these objects give an identification of vertices incident on each matched edge which can be pooled together without disconnecting the original graph, they are frequently used for coarsening.  To describe this more precisely, recall that a matching $\mathcal{M}$ is \emph{maximal} provided every edge in $\mathcal{G}$ has at least one of its endpoints matched, or equivalently provided no edges in $\mathcal{G}$ can be added to $\mathcal{M}$.  Note that maximal matchings are generally not unique, and could even contain different numbers of edges.  On the other hand, they can be computed easily through a simple greedy procedure which is $\mathcal{O}(|\mathcal{E}|)$, and also provide some control on the \emph{edge cut}, or number of edges which contain one matched and one unmatched vertex.  Heavy edge matching minimizes this quantity by greedily selecting the edges with greater weight, so that well separated regions of the graph are matched first.  While this is not guaranteed to produce a matching which minimizes the edge cut globally, it provides a fast and simple procedure which works well in practice.  Representative pseudocode is given in Algorithm~\ref{alg:heavyedge}.

% In particular, the vertices $v_i \in \mathcal{V}$ are visited in random order.  For each unmatched vertex $v_j$ adjacent to $v_i$, the values of $w_{ij}$ in the adjacency matrix are compared, and vertex $v_{j_0}$ (hence edge $e_{ij_0}$) is added to the matching provided $w_{ij_0} > w_{ij}$ for all relevant $j$. 


% has at least one neighboring vertex which is unmatched, 

\begin{algorithm}
\SetAlgoLined
\KwResult{Heavy edge matching $\mathcal{M}$ of the graph $\mathcal{G}$. }
 Initialize: empty list $\mathcal{M}$ of edges\;
\For{unmatched vertices $v_i \in \mathcal{V}$}{
    \For{unmatched vertices $v_j$ adjacent to $v_i$}{
        Determine vertex $v_{j_0}$ corresponding to largest normalized edge weight $w_{ij} / \max\{d_{ii}, d_{jj}\}$\;
    }
    Add $e_{ij_0}$ to $\mathcal{M}$ and mark $v_{j_0}$ as matched\;
}
\caption{Heavy Edge Matching}
\label{alg:heavyedge}
\end{algorithm}

Once a heavy edge matching $\mathcal{M}$ is computed, the graph $\mathcal{G}$ is coarsened by collapsing the edges $e_{ij}\in\mathcal{M}$ and pooling together matched nodes.  Following the notation of \cite{loukas2019}, the reduction of vertices when coarsening the graph $\mathcal{G}_{\ell-1}$ is formally captured by a surjective mapping of vertices $\phi_\ell: \mathcal{V}_{\ell-1} \to \mathcal{V}_\ell$ where the contraction set of node $v_r \in \mathcal{V}_\ell$ is given by $\mathcal{V}^r_{\ell-1} = \{ v\in\mathcal{V}_{\ell-1}\,:\,\phi_\ell(v) = v_r \}$.  It follows that the matrices $\bb{P}_\ell, \bb{P}^+_\ell$ take the componentwise form
\begin{align*}
    P_{\ell,ri} = 
    \begin{cases}
        \frac{1}{\nn{\mathcal{V}^r_{\ell-1}}} & v_i \in \mathcal{V}^r_{\ell-1}, \\
        0 & \mathrm{otherwise}.
    \end{cases} \qquad\qquad
    P^+_{\ell,ir} = 
    \begin{cases}
        1 & v_i \in \mathcal{V}^r_{\ell-1}, \\
        0 & \mathrm{otherwise}.
    \end{cases}
\end{align*}

This gives an explicit form for the coarsening (resp. lifting) of signals on $\mathcal{G}_{\ell-1}$ (resp. $\mathcal{G}_\ell$).   For example, if $\bb{x}_{(\ell-1),i}, \bb{x}_{(\ell-1),j}$ are signals at two nodes $v_i, v_j \in \mathcal{V}_{\ell-1}$ connected by the matched edge $e_{ij}$, the aggregated signal at the node $v_r \in \mathcal{V}_{\ell}$ formed by collapsing $e_{ij}$ is given by $\bb{x}_r=(\bb{x}_i + \bb{x}_j)/2$.  Moreover, note that if both $w_{ik}$ and $w_{jk}$ are nonzero in the adjacency matrix $\bb{A}_{\ell-1}$ so that both $v_i, v_j$ are connected to node $v_k$, then the corresponding entry in $\bb{A}_\ell$ is at least the sum $w_{ik} + w_{jk}$ (depending on the contraction set containing $v_k$).


% is weighted according to the sum of 

% Note that edges which are overlapped due to the contraction of nodes have their weights added together

% ``Laplacian-consistent coarsening'' method of \cite{loukas}.  In particular, we consider a scheme such that the combinatorial Laplacian of each subgraph is generated by simply projecting the combinatorial Laplacian of its parent, i.e. $\bb{L}_{\ell} = \bb{P}_\ell^\mp\bb{L}_{\ell-1}\bb{P}_\ell^+$.  It follows that ........


% Using this, it is not difficult to see that $\bb{\Pi} = \bb{P}_\ell^+\bb{P}_\ell$ is a projection matrix (since $\bb{\Pi}^2 = \bb{\Pi}$) and 

\textcolor{red}{this is probably dead at this point...}
Precisely, the authors of \cite{defferrard2016} propose the use of Chebyshev polynomials in the normalized Laplacian $\bb{L} = \bb{I} - \bb{D}^{-1/2}\bb{A}\bb{D}^{-1/2}$, and demonstrate their viability as GNN kernels.  Recall that the Chebyshev polynomials form a basis for $L^2\left([-1,1]\right)$ and satisfy the stable recurrence relation $T_k(x) = 2xT_{k-1}(x) - T_{k-2}(x)$ where $T_0(x) = 1$ and $T_1(x) = x$.  Writing $\bb{W} = g_\theta(\bb{L})$, this leads to the ChebNet convolution at layer $\ell$,
\begin{equation}\label{eq:chebconv}
    \bb{x}_{\ell,i} = \sig_\ell\left(\sum_{j=1}^{C_{in}} \bb{W}^j_{\ell,i} \bb{x}_{(\ell-1),j} + \bb{b}_{\ell,i} \right),
\end{equation}
where $\bb{x}_{\ell,i}$ denotes the $i^{th}$ output channel of the signal $\bb{x}_\ell$, the expressions $\bb{W}_{\ell,i}^j = \left(g_\theta(\bb{L})\right)_{\ell,i}^{j} =  \sum_k \theta_{\ell,ki}^j T_k(\tilde{\bb{L}})$ contain the $C_{in} \times C_{out}$ vectors of learnable parameters $\theta_{\ell,i}^j \in \mathbb{R}^{K+1}$ which are updated during network training, and $\tilde{\bb{L}} = 2\bb{L}/\lambda_{\mathrm{max}} - \bb{I}$ is a simple affine transformation which ensures that the eigenvalues lie in $[-1,1]$.  

\subsection{Graph Convolutional Autoencoder}
With this technology in place, it is possible to define a convolutional autoencoder architecture which operates on graphical signals.  Consider a graph $\mathcal{G}_0 = \{\mathcal{V}_0, \mathcal{E}_0\}$ and successive coarsenings $\mathcal{G}_1 \supset ... \supset \mathcal{G}_m$ computed by heavy edge matching, such that $\mathcal{G}_\ell = \{\mathcal{V}_\ell, \mathcal{E}_\ell\}$ has adjacency matrix $\bb{A}_\ell$.  The present graph convolutional network is built by successively convolving and downsampling an input signal $\bb{x}_0\in\mathbb{R}^{{N_0} \times n_0}$, yielding a latent representation which is similarly upsampled and convolved in the decoding phase.  To describe this precisely, it is convenient to consider the encoder $E$ and decoder $D$ as built from blocks $E_\ell, D_\ell$ so that at each layer $1 \leq \ell \leq m$,
\begin{align*}
    \bar{\bb{x}}_{\ell-1} &= f_\ell(\bb{x}_{\ell-1}) \in \mathbb{R}^{N_{\ell-1} \times n_\ell} \\
    \bb{x}_\ell &= E_\ell({\bb{x}_{\ell-1}}) = \bb{P}_\ell\bar{\bb{x}}_{\ell-1} \in \mathbb{R}^{N_{\ell} \times n_\ell},
\end{align*}
where $f_\ell$ denotes the Chebyshev convolution \eqref{eq:chebconv}.  
In this way $\bb{x}_{\ell}$ is a signal on graph $\mathcal{G}_{\ell}$.  Similar to the conventional CNN, the final layer $E_{m+1}$ of the encoder is a fully connected linear layer with 
\begin{align*}
    \bar{\bb{x}}_{m} &= \mathrm{flatten}\,(\bb{x}_{m}) \in \mathbb{R}^{N_m * n_{m}} \\
    \bb{x}_{m+1} &= E_{m+1}(\bb{x}_{m}) = \sig_{m+1}\left( \bb{W}_{m+1}\bar{\bb{x}}_{m} + \bb{b}_{m +1}\right) \in \mathbb{R}^{n_{m+1}},
\end{align*}
where $\mathrm{flatten}(\bb{x}_m)$ denotes a transformation which stacks the $n_m$ columns sequentially into a long vector. 
Therefore, the encoder $E = E_{m+1} \circ ... \circ E_1$ maps an input sample $\bb{x}=\bb{x}_0 \in \mathbb{R}^{N_0 \times n_0}$ to an encoded representation $\bb{x}_m \in \mathbb{R}^{n_{m+1}}$.  Similarly, the first layer of the decoder is also fully connected and employs a transformation $\mathrm{reshape}(\bb{x})$ which is the inverse of flatten,
\begin{align*}
    \hat{\bb{x}}_{m+1} &= D_{m+1}(\bb{x}_{m+1}) = \sig_{m+1}\left( \bb{W}'_{m+1}\bar{\bb{x}}_{m+1} + \bb{b}'_{m+1}\right) \in \mathbb{R}^{N_{m}*n_m}, \\ \tilde{\bb{x}}_m &= \mathrm{reshape}\,(\hat{\bb{x}}_{m+1}) \in \mathbb{R}^{N_m \times n_{m}}.
\end{align*}
Following this, the rest of the decoder mimics the structure of the encoder in reverse, i.e. for $m \geq \ell \geq 1$,
\begin{align*}
    \hat{\bb{x}}_\ell &= \bb{P}^+_\ell\tilde{\bb{x}}_{\ell} \in \mathbb{R}^{N_{\ell-1} \times n_\ell} \\
    \tilde{\bb{x}}_{\ell-1} &= f_\ell(\hat{\bb{x}}_{\ell}) \in \mathbb{R}^{N_{\ell-1} \times n_{\ell-1}}.
\end{align*}
This yields $D = D_1 \circ ... \circ D_{m+1}$ mapping the encoded representation $\bb{x}_{m+1}$ to an approximation $\tilde{\bb{x}}_0 \approx \bb{x}_0$ of the original signal.  Note that in practice the input is typically a batch of signals $\bb{x}_0 \in \mathbb{R}^{n_B \times N_0 \times n_0}$ where $n_B$ is the batch size.  This is the case when $\bb{x}_0$ is a collection of PDE solution snapshots at various parameter configurations $(t,\mmu)$. 

As in \cite{fresca2021}, the graph autoencoder network $D\circ E$ is trained alongside a fully connected network $F = F_1 \circ ... \circ F_k$ which approximates the low-dimensional dynamics. The purpose of $F$ is to map the parameter space (of size $n_\mu + 1)$ into the latent space $\mathbb{R}^{n_{m+1}}$ in a way that $D\circ F$ approximates the unique trajectories $(t,\mmu) \mapsto \bb{u}(t, \mmu) \in \mathbb{R}^{N_0 \times n_0}$ associated to the PDE solution $\bb{u}$.  In accordance with this, the mappings $D,E,F$ are updated according to the loss
\begin{equation*}
    L(\bb{x}, \bb{p}) = \frac{1}{n_B}\left( \nn{\bb{x} - D\circ F(\bb{p})}^2 + \nn{E(\bb{x}) - F(\bb{p})}^2 \right),
\end{equation*}
where $\bb{x}\in \mathbb{R}^{n_B \times N_0 \times n_0}$ is the batched snapshot matrix and $\bb{p}\in\mathbb{R}^{n_B \times (n_\mu + 1)}$ is the batched vector of points in parameter space.
